A Hierarchical Bayesian Model for Deep Few-Shot Meta Learning

We propose a novel hierarchical Bayesian model for learning with a large (possibly infinite) number of tasks/episodes, which suits well the few-shot meta learning problem. We consider episode-wise random variables to model episode-specific target generative processes, where these local random variables are governed by a higher-level global random variate. The global variable helps memorize the important information from historic episodes while controlling how much the model needs to be adapted to new episodes in a principled Bayesian manner. Within our model framework, the prediction on a novel episode/task can be seen as a Bayesian inference problem. However, a main obstacle in learning with a large/infinite number of local random variables in online nature, is that one is not allowed to store the posterior distribution of the current local random variable for frequent future updates, typical in conventional variational inference. We need to be able to treat each local variable as a one-time iterate in the optimization. We propose a Normal-Inverse-Wishart model, for which we show that this one-time iterate optimization becomes feasible due to the approximate closed-form solutions for the local posterior distributions. The resulting algorithm is more attractive than the MAML in that it is not required to maintain computational graphs for the whole gradient optimization steps per episode. Our approach is also different from existing Bayesian meta learning methods in that unlike dealing with a single random variable for the whole episodes, our approach has a hierarchical structure that allows one-time episodic optimization, desirable for principled Bayesian learning with many/infinite tasks. The code is available at \url{https://github.com/minyoungkim21/niwmeta}.

==> tmp/formatting.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\finalversion{0}
\newcommand{\finalVersion}{\def\finalversion{1}}

\usepackage[framemethod=tikz]{mdframed}
\usepackage{geometry}
\usepackage[many]{tcolorbox}
\usepackage{marginnote}

\newcounter{mynote}
\newtcolorbox[use counter=mynote]
  {mynote}[1][]
  {title=ToDo~\thetcbcounter,
   width=1.3in, %\marginparwidth,
   left=0pt,
   right=0pt,
   fonttitle=\bfseries\color{black},
   colframe=pink,
   colback=pink!10,
   #1
}

\newcommand\ToDo[2][]{%
  \colorbox{pink}{\small Todo}
  \marginnote[#1]{%
    \makebox[0pt][l]{\begin{mynote}[]
    \small #2
    \end{mynote}}}%
}

\newcommand\ToDoRef[3][]{%
  \colorbox{pink}{\small Todo:~\ref{#3}}
  \marginnote[#1]{%
    \makebox[0pt][l]{\begin{mynote}[label=#3]
    \small #2
    \end{mynote}}}%
}

\newcommand{\todo}[1]{\colorbox{pink}{\small Todo:#1}}
%\newcommand{\todo}[1]{\colorbox{pink}{Todo:#1}}
\newcommand{\todocite}[1]{\colorbox{red}{[??#1??]}}
\newcommand{\reviewerCommant}[1]{\textcolor{red}{Comment:#1}}
\newcommand{\solicitation}[1]{\if\finalversion1 {} \else \begin{mdframed}[hidealllines=true,backgroundcolor=blue!20]From Solicitation: \textit{#1}\end{mdframed} \fi}


==> tmp1.tex <==
We consider {\em learning with infinite tasks/episodes}, which can be formally stated as follows: $P(\mathcal{T})$ is the (unknown) task distribution, where each task $\mathcal{T} \sim P(\mathcal{T})$ is defined as a distribution $P_\mathcal{T}(x,y)$ for data $(x,y)$ where $x$ is input and $y$ is target. By episodic learning, we have an infinite number of tasks, $\mathcal{T}_1,\mathcal{T}_2,\dots, \mathcal{T}_N, \dots \sim P(\mathcal{T})$ sampled i.i.d., but we only observe a finite number of samples from each task/episode, denoted by $D_i = \{(x^i_j,y^i_j)\}_{j=1}^{n_i} \sim P_{\mathcal{T}_i}(x,y)$, where $n_i=|D_i|$ is the number of samples in $D_i$. 
The goal of the learner, after observing the training data $D_1,\dots,D_N,\dots$ from a large amount of tasks, is to build a predictor $p^*(y|x)$ for a novel unseen task $\mathcal{T}^*\sim P(\mathcal{T})$. We will often abuse the notation, e.g., $i\sim\mathcal{T}$ refers to the episode $i$ sampled, i.e., $D_i\sim P_{\mathcal{T}_i}(x,y)$ where $\mathcal{T}_i \sim P(\mathcal{T})$.
%
The {\em few-shot meta learning}~[CITE] is one of the best examples in this setup; in particular, at test time we are allowed to have some hints about the new test task $\mathcal{T}^*$, in the form of a few labeled examples from $\mathcal{T}^*$, also known as the support set\footnote{
For training data, we are typically given two labeled sets in the few-shot learning, {\em support} and {\em query}. Although many approaches use the support set for adaptation and measures the quality of the adapted model on the query set to get learning signals, we do not explicitly distinguish the two in our derivations. That is, we treat the union of the query and support sets as $D_i$. 
}. %\footnote{Although in meta learning it is popular to hold out a portion of the training data $D_i$ as a support set (and the rest as a query set), we do not explicitly consider this splitting in training data, but treat $D_i$ as a whole.}. 
For test data, only a support set is accessible, denoted by $D^*\sim P_{\mathcal{T}^*}(x,y)$.
 

In Bayesian perspective, the goal is to infer the posterior distribution with the (possibly infinite number of) training data as evidence, that is, $p(y|x,D_1,\dots,D_N,\dots)$. However, one major computational constraint is that the infinite number of tasks/data cannot be stored and hardly revisited, which implies that any viable learning algorithm has to be an {\em online algorithm} in nature. 






%%%%
\begin{itemize}
%
\item Few-shot classification
    \begin{enumerate}
    \item Standard benchmark comparisons on ResNet-18 and WideResNet backbones: (a) {\em mini}Imagenet Table~\ref{tab:mini}, (b) {\em tiered}ImageNet Table~\ref{tab:tiered}, (c) CIFAR-FS -- \hl{TODO: require dataloader impl...}
    \item Large-scale ViT backbones Table~\ref{tab:vit}: (a) {\em mini}Imagenet, (b) {\em tiered}ImageNet, (c) CIFAR-FS
    \item Error Calibration (ECE): Conv-4 and WRN on {\em mini}ImageNet Table~\ref{tab:ece_mini}
    \item Comparison with the set-based adaptation architectures, namely $y^Q = g(x^Q,S;\theta)$ that takes the entire support set $S$ and query input $x^Q$ as input to the network (e.g., FEAT~\cite{feat}): Our approach can incorporate any backbone network architecture, even set-based one like FEAT; Table~\ref{tab:feat}
    \item Meta-Dataset (comparison with SUR, URT, and MetaQDA): \hl{TODO}
    \item Cross-Domain experiments (e.g., mini$\to$CUB or mini$\to$Cars) : \hl{Perhaps, no cross-domain experiments done since it violates our model/data assumptions where the meta training data and meta test data follow the same task distribution!}
    \end{enumerate}
%
\item Few-shot regression
    \begin{enumerate}
    \item (Synthetic) SineLine (1D $(x,y)$ randomly generated by either linear or sine curves with different scales/slopes/frequencies/phases with $k=5$-shot support and $kq=45$ query samples): We introduce so called \textbf{RidgeNet} that has a parameter-free head derived from support data via (closed-form) estimation of the linear coefficient matrix using the ridge regression. So it is analogous to the ProtoNet in few-shot classification that also has a parameter-free head that is derived from the Gaussian linear discrimination analysis on support data.
    The RidgeNet leads to much more accurate prediction than conventional linear head whose parameters are trained for each episode, e.g., on SineLine dataset the test errors are: RidgeNet $=0.82$ vs.~linear head $=4.3$.
    Consequently, we can adopt the ridge head in other models as well, such as MAML, PMAML~\cite{platipus}, and our NIW-Meta. 
    See Table~\ref{tab:sineline} for the mean squared errors of the standard few-shot regression methods and our NIW-Meta.  
    The table also contains the regression-ECE (R-ECE) calibration errors (\hl{Put definition for R-ECE}) for the Bayesian methods, PMAML~\cite{platipus} and ours. 
    %
    \item ShapeNet datasets Table~\ref{tab:shapenet}: (a) Pascal-1D, (b) ShapeNet-1D, (c) ShapeNet-3D, (d) Distractor
    \end{enumerate}
%
\end{itemize}
%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Crucial Points to Address}


\begin{enumerate}
%%%%
%%%%
\item {\em \textcolor{blue}{ What is the unique selling point it can offer beyond Bayesian MAML and Probabilistic MAML etc?}} 
%
\\ \hl{How it is different from other Bayesian methods?}
The Probabilistic MAML (PMAML or Platipus)~\cite{platipus} has the same hierarchical graphical model structure as ours, but their learning algorithm is considerably deviated from the original variational inference objective. For instance, the KL term should measure divergence between the posterior and prior on the task-specific variable $\theta_i$, namely $\mathbb{E}_{q(\phi)}[\textrm{KL}(q_i(\theta_i|\phi) || p(\theta_i|\phi))]$
as in (\ref{eq:elbo_infinite}). But in PMAML, they measure the divergence on the global variable $\phi$, aiming to align the two adapted models, one from the support data only $q(\phi|S_i)$ and the other from both support and query $q(\phi|S_i,Q_i)$.
The Bayesian MAML (BMAML)~\cite{bmaml} is not a hierarchical Bayesian model, but mainly about replacing MAML's gradient-based (deterministic) adaptation steps by the probabilistic counterpart using the samples (aka particles) from the distribution $p(\theta_i|S_i)$ via the Stein variational gradient descent~[CITE] (thus adopting stochastic ensemble-based adaptation steps). If we use a single particle instead, it reduces exactly to MAML. Thus not directly related to our hierarchical Bayesian perspective. \tim{That's great to clarify! How about: AISTATS22: Is Bayesian Model-Agnostic Meta Learning Better than Model-Agnostic Meta Learning, Provably?}



%%%%
%%%%
\item {\em \textcolor{blue}{ Is there any practical benefit of the very different inference algorithm? EG: Focus on the fact that it gives a first order solution and with no storing of long compute graphs. Then we should compare to Reptile (\url{https://openai.com/blog/reptile/}) and other fast versions of MAML and show that it has a better accuracy/scalability tradeoff to them.}}
%
\\ \hl{Answer to relation to Reptile:} 
We have seen that ProtoNet can be seen as a special case of our approach: If we ignored the negative log-likelihood term when solving (\ref{eq:elbo_optim_mi}), the optimal solution becomes $m_i^*(L_0) = m_0$. This makes the last term of (\ref{eq:fi}) vanish, and $m_0$ updated only by gradient descent with $\nabla_{m_0}(-\log p(D_i|m_0))$, which reduces to the ProtoNet update if we use a parameter-free classification head (e.g., NCC). Now, if we ignored the quadratic penalty term in (\ref{eq:elbo_optim_mi}), then $m_i^*(L_0) = \overline{m}_i$ which is constant with respect to $L_0 = (m_0,V_0,n_0)$. This makes the ultimate optimization (\ref{eq:ultimate_optim}) very simple, where the optimal $m_0$ is the average of $\overline{m}_i$ for all tasks $i$, that is, $m_0^* = \mathbb{E}_{i \sim \mathcal{T}}[\overline{m}_i]$. Recall that Reptile ultimately finds the exponential average of $m_i^{(k)}$ over $i\sim \mathcal{T}$ where $m_i^{(k)}$ is the iterate after $k$ SGD steps for task $i$. This is a (popular) moving average solution for the estimate of $\mathbb{E}_{i \sim \mathcal{T}}[\overline{m}_i]$. Thus Reptile is also a special case of our approach. 
%%%%
%%%%
\item {\em \textcolor{blue}{A related point is that nobody ever seems to be able to make MAML work correctly on medium-big network architectures. IE: All MAML papers are <= ResNet18. ResNet50+ don't work. I don't think anyone knows why this empirical phenomenon happens. But it's possible your novel VI algorithm is better in this regard than the standard reverse mode/implicit gradient compute graph. If your HB-MAML Can really make big CNNs/transformers play well with MAML, that could be very influential.}}
%
\\ \hl{Answer:}
Ours work nicely with complex backbones including Vision Transformers (ViT)...
%%%%
%%%%
\item {\em \textcolor{blue}{ As we discussed, maybe in the non-spiky version where the posterior has learned variance, the ProtoNet special case ends up with a different feature extractor learning algorithm that could improve vanilla ProtoNet? If so would be interesting.}}
%
\\ \hl{Answer:} 
With the non-spiky version $q_i(\theta_i; L_i) = \mathcal{N}(\theta_i; m_i,V_i)$ (note: now $L_i=\{m_i,V_i\}$ and $V_i$ is learnable), there are a few modifications. First, (\ref{eq:eqphi_kl}) is changed to:
\begin{align}
&\mathbb{E}_{q(\phi)}\big[\textrm{KL}(q_i(\theta_i) || p(\theta_i|\phi))\big] \ = \label{eq:eqphi_kl_vi} \\
&\ \ \ \ \ \  \frac{n_0}{2} (m_i - m_0)^\top V_0^{-1} (m_i - m_0) + \frac{n_0}{2}\textrm{Tr}(V_0^{-1}V_i) - \frac{1}{2} \log |V_i| + \textrm{const.~w.r.t.~$L_i$}, \nonumber
\end{align}
and (\ref{eq:elbo_optim_mi}) becomes (we no longer have $\mathbb{E}_{q_i(\theta_i;L_i)}[-\log p(D_i|\theta_i)] \approx -\log p(D_i|m_i)$):
\begin{align}
\min_{m_i,V_i} \ &\Bigg( \mathbb{E}_{\mathcal{N}(\theta_i;m_i,V_i)}[-\log p(D_i|\theta_i)] + \frac{n_0}{2} (m_i - m_0)^\top V_0^{-1} (m_i - m_0) \nonumber \\
& \ \ \ \ \ \ + \frac{n_0}{2}\textrm{Tr}(V_0^{-1}V_i) - \frac{1}{2} \log |V_i| \Bigg).
\label{eq:elbo_optim_mi_vi}
\end{align}
So, if we use the same ProtoNet-special-case treatment (i.e., ignoring the expected negative log-likelihood term in (\ref{eq:elbo_optim_mi_vi})), then the optimal $(m_i,V_i)$ becomes:
\begin{align}
m_i^*(L_0) = m_0, \ \ \ \ V_i^*(L_0) = n_0^{-1}V_0.
\end{align}
Then if we plug this into (\ref{eq:elbo_optim_orig}), we have an optimization problem over a single variable $L_0=\{m_0,V_0,n_0\}$ as follows (as a counterpart of (\ref{eq:ultimate_optim})'s spiky version): 
\begin{align}
\min_{L_0} \ \ & \mathbb{E}_{i\sim\mathcal{T}} \Big[ \mathbb{E}_{\mathcal{N}(\theta_i; m_0,n_0^{-1}V_0)}[-\log p(D_i|\theta_i)] \Big] - \frac{1}{2} \psi_d\Big(\frac{n_0}{2}\Big) + \frac{d}{2} \log n_0. 
\label{eq:protonet_special_case_non_spiky}
\end{align}
If we use the multivariate digamma approximation $\psi_d(x) \approx d (\log x - 1/(2x))$, the last two terms reduces to $d/(2n_0)$ up to constant, yielding:
\begin{align}
\min_{L_0} \ \ & \mathbb{E}_{i\sim\mathcal{T}} \Big[ \mathbb{E}_{\mathcal{N}(\theta_i; m_0,n_0^{-1}V_0)}[-\log p(D_i|\theta_i)] \Big] +  \frac{d}{2n_0}. 
\label{eq:protonet_special_case_non_spiky_approx}
\end{align}
Then the ProtoNet special case for a non-spiky model becomes the following algorithm:
\begin{align}
&\ \ \ \ \textrm{(a) Sample} \ i \sim\mathcal{T}. \\
&\ \ \ \ \textrm{(b)} \ L_0 \leftarrow L_0 - \eta \nabla_{L_0} \bigg( \mathbb{E}_{\mathcal{N}(\theta_i; m_0,n_0^{-1}V_0)}[-\log p(D_i|\theta_i)] + \frac{d}{2n_0} \bigg).
\label{eq:protonet_special_case_non_spiky_alg}
\end{align}
If we send $n_0\to\infty$, then obviously  (\ref{eq:protonet_special_case_non_spiky_alg}) exactly coincides with the ProtoNet update. But if we update $n_0$ and $V_0$ together with $m_0$, then the algorithm can be seen as a {\em stochastic} extension of ProtoNet, namely we perturb the model parameters $m_0$ as per the covariance $n_0^{-1}V_0$ in ProtoNet query loss computation, where this covariance is optimized as well (neither growing indefinitely or vanishing completely due to the trade-off effect in both terms -- does this make sense? need to check it). Another note: If $f(\theta) := -\log p(D|\theta)$ is a convex function, then since $\mathbb{E}_\theta[f(\theta)] \geq f(\mathbb{E}[\theta]) = f(m_0)$, the first term of (\ref{eq:protonet_special_case_non_spiky}) becomes independent of $n_0$, and $n_0 \to \infty$ is optimal. So, it reduces to ProtoNet exactly. But if $f(\theta)$ is not convex, maybe not, but I guess $n_0 \to \infty$ is still near optimal.
%%%%
%%%%
\item {\em \textcolor{blue}{ Could compare the convergence and generalisation analysis from FedHB, which presumably can generalise to here(?) and see if they are favourable or not compared to existing convergence and generalisation analysis for MAML?}}
%
\\ \hl{Answer:} As our learning is an unbiased SGD over the infinite number of task batches, it should converge? but the question is how accurate the SGLD quadratic approximation of the task loss function is.
Regarding the generalisation error bound, we can immediately apply the FedHB's result without modification, but the question is the bound is meaningless if $n$ (size of each task data) is not large.
%%%%
%%%%
\item {\em \textcolor{blue}{ Maybe the decoupled algorithm makes it a good candidate for FederatedMAML? In that case need to study the existing FedMAML papers and figure out if/why we expect to be better. \url{https://proceedings.neurips.cc/paper/2020/file/24389bfe4fe2eba8bf9aa9203a44cdad-Paper.pdf}, \url{https://arxiv.org/abs/1909.12488} <-- Over 200 citations each so probably there are newer ones too.}}
%
\\ \hl{Answer:} Perhaps leave it as future work? but very soon?
%%%%
%%%%
\item {\em \textcolor{blue}{ Maybe if your HB-MAML can also use the mixture prior, then it could be a nice Bayesian solution to the mixture-of-MAML  challenge for when you have diverse datasets that prefer different initialisations (e.g., meta-dataset). Then we need to study the existing multi-initialisation MAMLs and figure out if/why we should be better \url{https://arxiv.org/abs/1905.05301}, \url{https://arxiv.org/abs/1910.13616}.}}
%
\\ \hl{Answer:} Perhaps leave it as future work? but very soon?
%%%%
%%%%
\item {\em \textcolor{blue}{ In practice MAML family methods that meta-learn the pre-conditioner, e.g., \url{https://arxiv.org/abs/1902.03356} perform very well in benchmarks. It seems unlikely, but not sure if there is any variant of your HB-MAML e.g., with full learned covariances, that can obtain a similar effect?}}
%
\\ \hl{Answer:} Perhaps leave it as future work? but very soon?
%%%%
%%%%
\item {\em \textcolor{blue}{ Do we want to directly compete Bayesian MAML + Probabilistic MAML etc in any of the typical reasons Bayesian models are good? EG: The regularisation from the prior. Or if our variant that learns an actual non-spiky Bayesian NN can work, then we could possibly compete on model calibration (cf: DKT, etc). But we discussed that can be tricky.}}
%
\\ \hl{Answer:} Non-spiky version is now available. We should measure the calibration performance.
%%%%
%%%%
\item {\em \textcolor{blue}{ This paper \url{https://arxiv.org/pdf/2205.10279.pdf} with LeCun and Wilson, mentioned that doing  SGLD-SWAG of Self-Supervision learns a very good posterior feature for various downstream tasks with. (And by the way they claim that the a real BNN with non-spiky Gaussian covariance is practically helpful, not just the mean, in contrast to your experience that it was tricky.) I wonder if there is any chance that learning a prior Gaussian feature with your method is even better than their SelfSup Gaussian feature. Because the Selfsup gaussian feature is only optimised for the pre-text task, which may or may not be good for downstream tasks. While your prior Gaussian feature is optimised to be a centroid of lots of practical tasks.}}
%
\\ \hl{???} I am not sure if this is what you originally meant, but inspired by your comments, how about tackling the self-supervised learning by forming infinitely many (or a large number of) supervised  tasks where the labels for each task are randomly generated? Then we may apply the current HB method to learn the feature extractor over these infinite random tasks. So, unlike popular self-sup methods that rely on a single data augmentation pretext task (eg, flipping an image preserves the class label), we may assign different (random) class labels for both original and augmented images. 
%%%%
%%%%
\item {\em \textcolor{blue}{ Intuition about continual learning.}}
%%%%
%%%%
\end{enumerate}

